IF-City: Intelligible Fair City Planning to Measure, Explain and Mitigate Inequality

With the increasing pervasiveness of Artificial Intelligence (AI), many visual analytics tools have been proposed to examine fairness, but they mostly focus on data scientist users. Instead, tackling fairness must be inclusive and involve domain experts with specialized tools and workflows. Thus, domain-specific visualizations are needed for algorithmic fairness. Furthermore, while much work on AI fairness has focused on predictive decisions, less has been done for fair allocation and planning, which require human expertise and iterative design to integrate myriad constraints. We propose the Intelligible Fair Allocation (IF-Alloc) Framework that leverages explanations of causal attribution (Why), contrastive (Why Not) and counterfactual reasoning (What If, How To) to aid domain experts to assess and alleviate unfairness in allocation problems. We apply the framework to fair urban planning for designing cities that provide equal access to amenities and benefits for diverse resident types. Specifically, we propose an interactive visual tool, Intelligible Fair City Planner (IF-City), to help urban planners to perceive inequality across groups, identify and attribute sources of inequality, and mitigate inequality with automatic allocation simulations and constraint-satisfying recommendations. We demonstrate and evaluate the usage and usefulness of IF-City on a real neighborhood in New York City, US, with practicing urban planners from multiple countries, and discuss generalizing our findings, application, and framework to other use cases and applications of fair allocation.

==> Requirement.tex <==
%!TEX root = FairPlannerTVCG.tex
\section{IF-City: Background}



Value-driven design through participatory preference elicitation.
Alternative methods include conducting workshops with residents, business owners, grassroots leaders, activists, ..., but that is time consuming and not scalable. Our approach complements this.

Using the IF-City tool falls within the planning phase where one or more urban designers/planners lay out aspects of the city such as building placements based on a design brief, compute metrics to evaluate against design criteria, and share the design artifacts for further discussion.

building types

resident types and preferences

\begin{figure*}
% \vspace{-0.5in}
\centering
\includegraphics[width=1\textwidth]{figures/FrontIMG.png}
\vspace{-0.25in}
\captionof{figure}{Fair Planner: {\color{red} make this figure simpler, left popup, building popup and city side bar} (A) 3D design dashboard where users can edit buildings. (B1), (B2) and (B3) show planning goals, background map and land use proportions. (C) Population Indicators shows occupancy and preference of each resident type. (D1) and (D2) plots the benefits and inequality scores of each resident type; Users can see where residents live and what are their benefit in 3D map using (D3) and (D4); (D5) shows benefit heatmap and occupancy cylinders on the map while buildings are hided. (E1) and (E2) provide editing preference settings and recommendations on mitigating inequality by editing certain blocks. (F) shows the comparisons of planning and inequality indicators of each editing version.
\label{fig:systemArchitecture}}
\end{figure*}




























